Flexible latent variable models on graphs: Laplace approximated inference for multiview network data

We propose a novel and flexible nonlinear approach for dimensionality reduction of large-scale multiview network data and derive its theory. The (linear) predictor incorporates observed covariates (edge-specific, layer-specific, and global) and Gaussian latent factors. Inference is conducted via the graph Laplace approximated maximum likelihood estimator. Letting $K$ denote the number of network layers and $n_V$ the number of nodes, we derive asymptotic theory under two regimes: (i) $K \to \infty$ with fixed $n_V$, and (ii) double asymptotics $K, n_V \to \infty$, establishing consistency and asymptotic normality for local and global parameters, with distinct convergence rates. In an application to the gravity model for commodity trades, we use a zero-adjusted Gamma distribution with latent factors and observable covariates (e.g.\ distance, tariffs, common language) to capture excess zeros, skewness, and unobserved heterogeneity. Synthetic and real-data exercises show that our approach outperforms the routinely applied Poisson pseudo-maximum likelihood estimator with fixed effects. We complement our theoretical and empirical contributions with open-source R/C++ routines and a novel strategy for starting values selection.

==> AnnasCommands.tex <==
\providecommand*{\definitionautorefname}{Definition}

\RequirePackage[OT1]{fontenc}
\numberwithin{equation}{section}
\hypersetup{
    colorlinks,%
    citecolor=blue,%
    filecolor=red,%
    linkcolor=blue,%
    urlcolor=blue
} 

% Autoref setup
\makeatletter
% Source - https://tex.stackexchange.com/a/183682
% Posted by user30471, modified by community. See post 'Timeline' for change history
% Retrieved 2026-04-24, License - CC BY-SA 3.0
% define a macro \Autoref to allow multiple references to be passed to \autoref
\newcommand\Autoref[1]{\@first@ref#1,@}
\def\@throw@dot#1.#2@{#1}% discard everything after the dot
\def\@set@refname#1{%    % set \@refname to autoefname+s using \getrefbykeydefault
    \edef\@tmp{\getrefbykeydefault{#1}{anchor}{}}%
    \xdef\@tmp{\expandafter\@throw@dot\@tmp.@}%
    \ltx@IfUndefined{\@tmp autorefnameplural}%
         {\def\@refname{\@nameuse{\@tmp autorefname}s}}%
         {\def\@refname{\@nameuse{\@tmp autorefnameplural}}}%
}
\def\@first@ref#1,#2{%
  \ifx#2@\autoref{#1}\let\@nextref\@gobble% only one ref, revert to normal \autoref
  \else%
    \@set@refname{#1}%  set \@refname to autoref name
    \@refname~\ref{#1}% add autoefname and first reference
    \let\@nextref\@next@ref% push processing to \@next@ref
  \fi%
  \@nextref#2%
}
\def\@next@ref#1,#2{%
   \ifx#2@ and~\ref{#1}\let\@nextref\@gobble% at end: print and+\ref and stop
   \else, \ref{#1}% print  ,+\ref and continue
   \fi%
   \@nextref#2%
}


\setlength{\textwidth}{17cm}
\setlength{\textheight}{22cm} \setlength{\oddsidemargin}{-.4cm}
\setlength{\topmargin}{-10mm}

% Colors
\def\Red{\special{color cmyk 0 1. 1. 0}} % PANTONE RED
\def\Black{\special{color cmyk 0 0 0 1.}} % PANTONE PROCESS-BLACK
\def\Green{\special{color cmyk 0.64 0 0.95 0.55}} % PANTONE 582
\def\Blue{\special{color cmyk 1. 1. 0 0}} % PANTONE BLUE-072

\DeclareMathOperator{\plim}{plim}

\renewcommand{\r}{\right}
\renewcommand{\l}{\left}
\long\def\symbolfootnote[#1]#2{\begingroup\def\thefootnote{\fnsymbol{footnote}}\footnote[#1]{#2}\endgroup}

\newcommand{\bb}{\boldsymbol{\beta}}
\newcommand{\bij}{\boldsymbol{\beta}_{ij}}
\newcommand{\db}{\frac{\partial }{\partial \bij}}
\newcommand{\dtl}{\frac{\partial }{\partial \theta_l}}
\newcommand{\gf}[1][\bzhk]{\Gamma\left(\bt, \bxx,\bw, #1 \right)}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% commands for faster typing 
% Response
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\byk}{\by^{(k)}}
% Density
\newcommand{\fa}{f_{\boldsymbol{\alpha}, \boldsymbol{\beta}}(\by)}
\newcommand{\fat}{\tilde{f}_{\boldsymbol{\alpha}}\left(\boldsymbol{y}^{(k)}\right)}
\newcommand{\fabg}[1]{f_{\baa, \sigma, \bb, \bg} \left(\by^{#1} \right)}
\newcommand{\tdens}{\tilde{f}_{\bt}\left(\byk\right)}
\newcommand{\dens}{f_{\bt}\left(\byk\right)}
% LV's
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bzh}{\hat{\mathbf{z}}}
\newcommand{\bZ}{\mathbf{Z}}
\newcommand{\bZt}{\mathbf{Z}_{(2)}}
\newcommand{\bzt}{\mathbf{z}_{(2)}}
\newcommand{\bztk}{\mathbf{z}_{(2)}^{(k)}}
\newcommand{\bZtk}{\mathbf{Z}_{(2)}^{(k)}}
\newcommand{\bzth}{\hat{\mathbf{z}}_{(2)}}
\newcommand{\bztht}{\hat{\mathbf{z}}_{(2)}^{\top}}
\newcommand{\bztkh}{\hat{\mathbf{z}}_{(2)}^{(k)}}
\newcommand{\bzhk}{\hat{\mathbf{z}}^{(k)}}
\newcommand{\bztkt}{\mathbf{z}_{(2)}^{(k)^{\top}}}
\newcommand{\bzk}{\mathbf{z}^{(k)}}
% Factor loadings (alpha)
\newcommand{\baa}{\boldsymbol{\alpha}}
\newcommand{\baat}[1][]{\baa_{(2) #1}}
\newcommand{\baath}[1][]{\hat{\baa}_{(2) #1}}
\newcommand{\aij}{\boldsymbol{\alpha}_{ij}}
\newcommand{\ac}[1][F]{\baa_{0, \mathcal{#1}}}
\newcommand{\ach}[1][F]{\hat{\baa}_{0, \mathcal{#1}}}
% Zeta
\newcommand{\bze}{\boldsymbol{\zeta}}
% Covariates: X (layer-dependent)
\newcommand{\bxx}{\mathbf{x}}
\newcommand{\xijk}{\bxx_{ij}^{(k)}}
% Covariates: W (layer-independent)
\newcommand{\bw}{\mathbf{w}}
% corresponding design matrix: W (layer-independent)
\newcommand{\bW}{\mathbf{W}}
% Linear predictor (eta)
\newcommand{\be}{\boldsymbol{\eta}}
\newcommand{\beij}{\be_{ij}}
\newcommand{\beijk}{\be_{ij}^{(k)}}
\newcommand{\eijk}{\eta_{ij}^{(k)}}
\newcommand{\eijkh}{\hat{\eta}_{ij}^{(k)}}
% s = a0 + Wg
\newcommand{\bs}{\boldsymbol{s}}
% mu
\newcommand{\bmu}[1][x]{\boldsymbol{\mu}_{#1}}
% Other parameters
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bp}{\boldsymbol{\pi}}
\newcommand{\bt}{\boldsymbol{\theta}}
\newcommand{\hbt}{\boldsymbol{\hat{\theta}}}
\newcommand{\vt}{{\vartheta}}
\newcommand{\vto}{\bvt_0}
\newcommand{\bvt}{\boldsymbol{\vt}}
\newcommand{\tvtkm}{\hat{\bt}}
\newcommand{\bpar}{\baa, \bb, \bg}
\newcommand{\ef}{\boldsymbol{\alpha}_{i j}^{\prime} \mathbf{z} + \mathbf{\beta}_{i j}^{\prime} \mathbf{x}}
\newcommand{\efzk}{\boldsymbol{\alpha}_{i j}^{\prime} \zhk + \mathbf{\beta}_{i j}^{\prime} \mathbf{x}}
\newcommand{\bx}{\boldsymbol{\xi}}
\newcommand{\bg}{\boldsymbol{\gamma}}

\newcommand{\ebe}{ \exp \left(\boldsymbol{\eta}\right) }
\newcommand{\aat}{ [\baa_{\boldsymbol{(2)}}]_{\cdot,ij} [\baa_{\boldsymbol{(2)}}]_{\cdot,ij}^{\top}}
\newcommand{\xfzk}{ \exp \left( - \exp \left( \efzk \right) \right) }
% Estimators
% z
\newcommand{\zhk}{\hat{\mathbf{z}}^{(k)}}
\newcommand{\zhkt}{\hat{\mathbf{z}}^{(k)^{\top}}}
%%%%%%%%%%% ZIG / ZAGA %%%%%%%%%%%%%%
\newcommand{\es}[1]{\eta_{#1}^k}
\newcommand{\elk}{\ell_{ij}^{(k)}}
\newcommand{\Yijk}{Y_{ij}^{(k)}}
\newcommand{\yijk}{y_{ij}^{(k)}}
\newcommand{\mij}{\mu_{ij}}
\newcommand{\mijk}{\mij^{(k)}}
\newcommand{\nij}{\nu_{ij}}
\newcommand{\nijk}{\nu_{ij}^{(k)}}
\newcommand{\pij}{\pi_{ij}}
\newcommand{\pijk}{\pij^{(k)}}
\newcommand{\qf}[1][, \bzk]{Q\left(\bt, \bxx, \bw #1, \byk\right)}
\newcommand{\uf}{U \left( \bt, \bzhk \right)}
\newcommand{\snv}{\sum_{i \neq j}^{n_V}}
\newcommand{\sk}{\sum_{k=1}^{K}}
\newcommand{\snmt}{\sum_{k=1}^{n_{m_{\tl}}}}
\newcommand{\nmt}{n_{m_{\tl}}}
\newcommand{\rmt}{r_{m_{\tl}}}
\newcommand{\eo}{\eta_{1, ij} = \ln \mij }
\newcommand{\eij}[1][]{\eta_{#1 ij} }
\newcommand{\mijex}{\exp (\eij{1})}
\newcommand{\et}{\eta_{2, ij} = \ln \nij }
\newcommand{\nijex}{\exp (\eij{2})}
\newcommand{\etath}{\eta_{3, ij} = \operatorname{logit} \pij }
\newcommand{\pijex}{\frac{\exp (\eij{3})}{1+\exp (\eij{3})}}
\newcommand{\lik}{\Biggl[  \ln\left\{ \pijk\right\} I_{\left( \yijk = 0 \right)} +\left[ \ln (1-p_{ij}) - \ln \Gamma (\mij) - \mij \ln (\nij) + (\mij -1) \ln (\yijk) - \yijk / \nij\right]   I_{\left( \yijk > 0 \right)} \Biggr]}

% indicator
\newcommand{\ind}[1]{\mathbbm{1} {\left( \yijk #1 0 \right)}}
\newcommand{\indo}[1]{\mathbbm{1} {\left( y_{ij} #1 0 \right)}}
% pi part of the log lik
\newcommand{\llp}{\ell_{\pi, ij}^{(k)}}
% gamma part of log lik
\newcommand{\llg}{\ell_{\bt, ij}^{(k)}}
% number of zero obs per layer
\newcommand{\noij}{n_{0,ij}}
\newcommand{\bigo}[1]{O\left(#1\right)}
\newcommand{\bigop}[1]{O_p\left(#1\right)}
\newcommand{\tl}{\theta}
\newcommand{\ts}{\theta^*}
\DeclareMathOperator{\vect}{vec}

\newcommand{\ThKM}{\Theta_{m}}
\newcommand{\bphi}{\boldsymbol{\varphi}}
\newcommand{\pKM}{p_{m}}
\newcommand{\pKMe}{p_{m}^E}
\newcommand{\pKMg}{p_{m}^G}
\newcommand{\delKM}{\delta^\infty_{K,m}}
\newcommand{\rKM}{r_{K,m}}
\newcommand{\Gamk}{\Gamma_k}
\newcommand{\zhatk}{\hat{\mathbf z}^{(k)}}
\newcommand{\rank}{\operatorname{rank}}

%score
\newcommand{\sco}[1][\tl]{\boldsymbol{S}^{(k)}(#1)}
\newcommand{\tsco}[1][\tl]{\tilde{\boldsymbol{S}}^{(k)}(#1)}
\newcommand{\Sco}[1][\bt]{\boldsymbol{\boldsymbol{\mathcal{S}}}^{(k)}(#1)}
\newcommand{\tSco}[1][\bt]{\tilde{\boldsymbol{\mathcal{S}}}^{(k)}(#1)}

% hessian
\newcommand{\hes}[1][\tl]{{H}_k(#1)}
\newcommand{\thes}[1][\tl]{\left. \partial_{\bt}^\T \partial_{\bt} \ln \tdens \right|_{\bt = #1}}
% \epsilon_k(\tl) = \ln ~f -\ln f, 
\newcommand{\epsk}[1][\tl]{\epsilon^{(k)}(#1)}
% \epsilon_d^k(\tl), per-level contribution
\newcommand{\epsd}[1][\tl]{\epsilon_d^{(k)}(#1)}
% \delta_k(\tl) = || d/d tl epsilon_k (\tl) ||
\newcommand{\delk}[1][\boldsymbol{\vt}]{\delta^{(k)} (#1) }
\newcommand{\Dvt}{D_{\vartheta}}
% sup


% \SupK[<k-range>][<theta-range>]
% - If the first optional argument is OMITTED, it defaults to 1 \le k \le K.
% - If the first optional argument is PRESENT but EMPTY (i.e., []), it is removed.
% - The second optional argument always defaults to \tl \in \mathcal{B}(\vto, t),
%   but can be overridden; it can also be set to empty via [].
\NewDocumentCommand{\SupK}{ o O{\tl \in \mathcal{B}(\theta_0, t)} }{%
  % Determine the k-part:
  \IfNoValueTF{#1}{\def\SupK@k{1 \le k \le K}}{\def\SupK@k{#1}}%
  % Cases:
  \ifstrempty{\SupK@k}{%
    \ifstrempty{#2}{%
      \sup
    }{%
      \sup_{\substack{#2}}%
    }%
  }{%
    \ifstrempty{#2}{%
      \sup_{\substack{\SupK@k}}%
    }{%
      \sup_{\substack{\SupK@k \\ #2}}%
    }%
  }%
}
%%%%%%%%%%%%%%%%%%%%%%%%%
\linespread{1.2}

%========================
% Norms
%========================
% Default vector norm
% Default matrix operator norm induced by \|\cdot\|_\infty
\newcommand{\mnorm}[1]{\left\|#1\right\|_{\infty}}

% Max-entry norm (used for tensors and for entrywise bounds)
\newcommand{\enorm}[1]{\left\|#1\right\|_{\max}}

% Spectral norm
\newcommand{\snorm}[1]{\left\|#1\right\|_{2}}

% Default inf norm
\newcommand{\norm}[1]{\left\|#1\right\|_{}}

% Balls are always defined using the default vector norm \|\cdot\|_\infty
\newcommand{\Ball}[2]{\mathcal{B}\left(#1,#2\right)}



